Multi-Modal Classifiers for Open-Vocabulary Object Detection

The goal of this paper is open-vocabulary object detection (OVOD) $\unicode{x2013}$ building a model that can detect objects beyond the set of categories seen at training, thus enabling the user to specify categories of interest at inference without the need for model retraining. We adopt a standard two-stage object detector architecture, and explore three ways for specifying novel categories: via language descriptions, via image exemplars, or via a combination of the two. We make three contributions: first, we prompt a large language model (LLM) to generate informative language descriptions for object classes, and construct powerful text-based classifiers; second, we employ a visual aggregator on image exemplars that can ingest any number of images as input, forming vision-based classifiers; and third, we provide a simple method to fuse information from language descriptions and image exemplars, yielding a multi-modal classifier. When evaluating on the challenging LVIS open-vocabulary benchmark we demonstrate that: (i) our text-based classifiers outperform all previous OVOD works; (ii) our vision-based classifiers perform as well as text-based classifiers in prior work; (iii) using multi-modal classifiers perform better than either modality alone; and finally, (iv) our text-based and multi-modal classifiers yield better performance than a fully-supervised detector.

==> assets/tables/lvis.tex <==
% !TEX root = ../../main.tex
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{@{}c|c|cc|ccc@{}}
\toprule
\setlength\tabcolsep{0pt}
Model                    & Backbone                   & $\mathset{D}{det}$?                  & $\mathset{D}{img}$?      & mAP           & APr           \\ \midrule
ViLD \cite{Gu2021}       & \multirow{6}{*}{ResNet-50} & \multirow{6}{*}{\textit{\checkmark}} & \multirow{6}{*}{\xmark}  & 22.5          & 16.1          \\
ViLD-ens \cite{Gu2021}   &                            &                                      &                          & 25.5          & 16.6          \\
F-VLM \cite{Kuo2022}     &                            &                                      &                          & 24.2          & 18.6          \\
Detic \cite{Zhou2022}    &                            &                                      &                          & 30.0          & 16.3          \\
Detic* \cite{Zhou2022}   &                            &                                      &                          & 29.7          & 15.6          \\
Ours                     &                            &                                      &                          & \textbf{30.3} & \textbf{19.3} \\ \midrule
RegCLIP \cite{Zhong2022} & \multirow{4}{*}{ResNet-50} & \multirow{4}{*}{\textit{\checkmark}} & \textit{CC3M}            & 28.2          & 17.1          \\
Detic \cite{Zhou2022}    &                            &                                      & \textit{IN-L}            & 32.4          & 24.6          \\
Detic* \cite{Zhou2022}   &                            &                                      & \textit{IN-L}            & 32.5          & 24.1          \\
Ours                     &                            &                                      & \textit{IN-L}            & \textbf{32.7} & \textbf{25.8} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}


==> assets/tables/lvis_cons.tex <==
% !TEX root = ../../main.tex

\begin{adjustbox}{width=\linewidth}
\begin{tabular}{@{}cccc|cc|cc@{}}
\toprule
% \setlength\tabcolsep{0pt}
\multicolumn{1}{c|}{\multirow{2}{*}{Vis. Enc.}} & \multicolumn{1}{c|}{\multirow{2}{*}{TTA?}} & \multicolumn{1}{c|}{\multirow{2}{*}{Agg.?}}      & \multirow{2}{*}{MM?}        & \multicolumn{2}{c|}{Training Data}                        & \multirow{2}{*}{mAP}     & \multirow{2}{*}{APr}     \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                            &                             & $\mathset{D}{det}$?         & $\mathset{D}{img}$?         &                          &                          \\ \midrule
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\xmark}}     & \multirow{3}{*}{\xmark}     & \multirow{6}{*}{\checkmark} & \multirow{6}{*}{\xmark}     & 28.8                     & 14.8                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 29.4                     & 17.3                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 28.8                     & 19.1                     \\ \cmidrule(r){1-4} \cmidrule(l){7-8} 
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\checkmark}} & \multirow{3}{*}{\xmark}     &                             &                             & 29.2                     & 18.3                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 26.6                     & 13.5                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 26.1                     & 11.7                     \\ \midrule
\multicolumn{4}{c|}{Text-based Classifiers}                                                                                                                                    & \checkmark                  & \xmark                      & \multicolumn{1}{l}{30.3} & \multicolumn{1}{l}{19.3} \\ \midrule
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\xmark}}     & \multirow{3}{*}{\xmark}     & \multirow{6}{*}{\checkmark} & \multirow{6}{*}{\checkmark} & 31.3                     & 21.6                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 31.6                     & 22.0                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 31.9                     & 24.1                     \\ \cmidrule(r){1-4} \cmidrule(l){7-8} 
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\checkmark}} & \multirow{3}{*}{\xmark}     &                             &                             & 31.3                     & 23.8                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & aa.b                     & aa.b                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & aa.b                     & aa.b                     \\ \midrule
\multicolumn{4}{c|}{Text-based Classifiers}                                                                                                                                    & \checkmark                  & \checkmark                  & \multicolumn{1}{l}{32.7} & \multicolumn{1}{l}{25.8} \\ \midrule
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\xmark}}     & \multirow{3}{*}{\checkmark} & \multirow{6}{*}{\checkmark} & \multirow{6}{*}{\xmark}     & 30.5                     & 20.7                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 29.8                     & 18.0                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 29.9                     & 19.3                     \\ \cmidrule(r){1-4} \cmidrule(l){7-8} 
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\checkmark}} & \multirow{3}{*}{\checkmark} &                             &                             & 30.6                     & 19.3                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 30.0                     & 18.3                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 29.6                     & 18.5                     \\ \midrule
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\xmark}}     & \multirow{3}{*}{\checkmark} & \multirow{6}{*}{\checkmark} & \multirow{6}{*}{\checkmark} & 32.8                     & 26.5                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & aa.b                     & aa.b                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & aa.b                     & aa.b                     \\ \cmidrule(r){1-4} \cmidrule(l){7-8} 
\multicolumn{1}{c|}{CLIP}                        & \multicolumn{1}{c|}{\checkmark}            & \multicolumn{1}{c|}{\multirow{3}{*}{\checkmark}} & \multirow{3}{*}{\checkmark} &                             &                             & 33.1                     & 27.3                     \\
\multicolumn{1}{c|}{Det-S}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 32.8                     & 26.4                     \\
\multicolumn{1}{c|}{Det-L}                       & \multicolumn{1}{c|}{\xmark}                & \multicolumn{1}{c|}{}                            &                             &                             &                             & 32.1                     & 23.3                     \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}



==> assets/tables/lvis_fused.tex <==
% !TEX root = ../../main.tex
\begin{table}[h!]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{@{}c|c|cc|ccc@{}}
\toprule
\setlength\tabcolsep{0pt}
Method                  & TTA?       & $\mathset{D}{det}$?                 & $\mathset{D}{img}$?            & mAP  & APr  \\ \midrule
Text + CLIP Baseline    & \checkmark & \multirow{6}{*}{\textit{LVIS-base}} & \multirow{6}{*}{$\varnothing$} & 30.5 & 20.7 \\
Text + Detic-S Baseline & \xmark     &                                     &                                & 29.8 & 18.0 \\
Text + Detic-L Baseline & \xmark     &                                     &                                & 29.9 & 19.3 \\ \cmidrule(r){1-2} \cmidrule(l){5-6} 
Text + Ours w/ CLIP     & \checkmark &                                     &                                & 30.6 & 19.2 \\
Text + Ours w/ Detic-S  & \xmark     &                                     &                                & aa.b & aa.b \\
Text + Ours w/ Detic-L  & \xmark     &                                     &                                & aa.b & aa.b \\ \midrule
Text + CLIP Baseline    & \checkmark & \multirow{6}{*}{\textit{LVIS-base}} & \multirow{6}{*}{\textit{IN-L}} & 32.8 & 26.5 \\
Text + Detic-S Baseline & \xmark     &                                     &                                & xx.y & xx.y \\
Text + Detic-L Baseline & \xmark     &                                     &                                & xx.y & xx.y \\ \cmidrule(r){1-2} \cmidrule(l){5-6} 
Text + Ours w/ CLIP     & \checkmark &                                     &                                & 33.1 & 27.3 \\
Text + Ours w/ Detic-S  & \xmark     &                                     &                                & xx.y & xx.y \\
Text + Ours w/ Detic-L  & \xmark     &                                     &                                & xx.y & xx.y \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\captionof{table}{
Results when using our method with fused templates,
comparing with equivalent simple baselines as done with image-based templates.
We use three types of models to an embedding from each template: CLIP, Detic-S and Detic-L.
See Section~\ref{ssec:results} for details on each of these models.
The use of test-time augmentation (TTA), or lack thereof, is indicated for each model.
We report mask AP metrics.
}\label{tab:lvis_fused}
\end{table}


==> assets/tables/lvis_img.tex <==
% !TEX root = ../../main.tex
\begin{table}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{@{}c|c|cc|ccc@{}}
\toprule
\setlength\tabcolsep{0pt}
Method                            & TTA?               & \multicolumn{1}{l}{$\mathset{D}{det}$?} & \multicolumn{1}{l|}{$\mathset{D}{img}$?} & mAP  & APr  \\ \midrule
\multirow{3}{*}{CLIP Baseline}    & \xmark             & \multirow{18}{*}{\textit{LVIS-base}}    & \multirow{18}{*}{$\varnothing$}          & 29.4 & 13.0 \\
                                  & \checkmark, harsh  &                                         &                                          & 29.5 & 15.1 \\
                                  & \checkmark, gentle &                                         &                                          & 29.8 & 14.8 \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Detic-L Baseline} & \xmark             &                                         &                                          & 28.8 & 19.1 \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & 28.4 & 16.2 \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Detic-S Baseline} & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Ours (CLIP)}      & \xmark             &                                         &                                          & 29.0 & 16.3 \\
                                  & \checkmark, harsh  &                                         &                                          & 29.0 & 17.2 \\
                                  & \checkmark, gentle &                                         &                                          & 29.2 & 18.3 \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Ours (Detic-L)}   & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Ours (Detic-S)}   & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \midrule
\multirow{3}{*}{CLIP Baseline}    & \xmark             & \multirow{18}{*}{\textit{LVIS-base}}    & \multirow{18}{*}{\textit{IN-L}}          & 31.6 & 22.5 \\
                                  & \checkmark, harsh  &                                         &                                          & 31.0 & 22.3 \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Detic-L Baseline} & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Detic-S Baseline} & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Ours (CLIP)}      & \xmark             &                                         &                                          & 31.4 & 22.7 \\
                                  & \checkmark, harsh  &                                         &                                          & 31.5 & 23.3 \\
                                  & \checkmark, gentle &                                         &                                          & 31.3 & 23.8 \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Ours (Detic-L)}   & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \cmidrule(r){1-2} \cmidrule(l){5-6}
\multirow{3}{*}{Ours (Detic-S)}   & \xmark             &                                         &                                          & -    & -    \\
                                  & \checkmark, harsh  &                                         &                                          & -    & -    \\
                                  & \checkmark, gentle &                                         &                                          & -    & -    \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\captionof{table}{Results when using image-based templates, comparing a simple CLIP baseline with our method.
We also report the effects of test-time augmentation (TTA) when generating the classifier embeddings.
We report mask AP metrics.
}\label{tab:lvis_img}
\end{table}


==> assets/tables/lvis_img2.tex <==
% !TEX root = ../../main.tex
\begin{table}[h!]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{@{}c|c|cc|ccc@{}}
\toprule
\setlength\tabcolsep{0pt}
Method           & TTA?       & $\mathset{D}{det}$?                 & $\mathset{D}{img}$?            & mAP  & APr  \\ \midrule
CLIP Baseline    & \checkmark & \multirow{6}{*}{\textit{LVIS-base}} & \multirow{6}{*}{$\varnothing$} & 28.8 & 14.8 \\
Detic-S Baseline & \xmark     &                                     &                                & 29.4 & 17.3 \\
Detic-L Baseline & \xmark     &                                     &                                & 28.8 & 19.1 \\ \cmidrule(r){1-2} \cmidrule(l){5-6} 
Ours w/ CLIP     & \checkmark &                                     &                                & 29.2 & 18.3 \\
Ours w/ Detic-S  & \xmark     &                                     &                                & aa.b & aa.b \\
Ours w/ Detic-L  & \xmark     &                                     &                                & aa.b & aa.b \\ \midrule
CLIP Baseline    & \checkmark & \multirow{6}{*}{\textit{LVIS-base}} & \multirow{6}{*}{\textit{IN-L}} & 31.3 & 21.6 \\
Detic-S Baseline & \xmark     &                                     &                                & 31.6 & 22.0 \\
Detic-L Baseline & \xmark     &                                     &                                & 31.9 & 24.1 \\ \cmidrule(r){1-2} \cmidrule(l){5-6} 
Ours w/ CLIP     & \checkmark &                                     &                                & 31.3 & 23.8 \\
Ours w/ Detic-S  & \xmark     &                                     &                                & xx.y & xx.y \\
Ours w/ Detic-L  & \xmark     &                                     &                                & xx.y & xx.y \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\captionof{table}{
Results when using our method for image-based templates, comparing with equivalent simple baselines.
We use three types of models to an embedding from each template: CLIP, Detic-S and Detic-L.
See Section~\ref{ssec:results} for details on each of these models.
The use of test-time augmentation (TTA), or lack thereof, is indicated for each model.
We report mask AP metrics.
}\label{tab:lvis_img}
\end{table}

